From Crowd Motion Prediction to Robot Navigation in Crowds

We focus on robot navigation in crowded environments. To navigate safely and efficiently within crowds, robots need models for crowd motion prediction. Building such models is hard due to the high dimensionality of multiagent domains and the challenge of collecting or simulating interaction-rich crowd-robot demonstrations. While there has been important progress on models for offline pedestrian motion forecasting, transferring their performance on real robots is nontrivial due to close interaction settings and novelty effects on users. In this paper, we investigate the utility of a recent state-of-the-art motion prediction model (S-GAN) for crowd navigation tasks. We incorporate this model into a model predictive controller (MPC) and deploy it on a self-balancing robot which we subject to a diverse range of crowd behaviors in the lab. We demonstrate that while S-GAN motion prediction accuracy transfers to the real world, its value is not reflected on navigation performance, measured with respect to safety and efficiency; in fact, the MPC performs indistinguishably even when using a simple constant-velocity prediction model, suggesting that substantial model improvements might be needed to yield significant gains for crowd navigation tasks. Footage from our experiments can be found at https://youtu.be/mzFiXg8KsZ0.

==> archived/OLD-prediction.tex <==




\section{Probabilistic Trajectory Prediction using SGANs}

Based on the formulation of probabilistic trajectory prediction models and recent works \citep{gupta2018social}, we use a state of the art approach, \textbf{Social GAN} to generate trajectory distribution predictions for crowd navigation.

A Generative Adversarial Network \citep{NIPS2014_GAN1}, consists of two neural networks: a generative model $\mathcal{G}$ that estimates the data distribution and the discriminative model $\mathcal{D}$ that estimates the probability that a sample
came from the training data rather than $\mathcal{G}$. The generator and discriminator are trained in a min-max game with the following objective:
\begin{equation}
\begin{aligned}
&\min _{G} \max _{D} V(G, D)= \\
&\mathbb{E}_{x \sim p_{\text {data }}(x)}[\log D(x)]+\mathbb{E}_{z \sim p_{(z)}}[\log (1-D(G(z)))]
\end{aligned}
\label{eq:gan}
\end{equation}

Given training data $\mathcal{D}_{train}$ with distribution $p(d\in\mathcal{D}_{train})$, and latent variable $z \sim \mathbf{N}(0, 1)$, the generator takes as input $z$ and outputs a sample in the training distribution i.e. $\mathcal{G}(z) \sim p(d)$. This formulation can be extended to conditional distributions such that given a condition $c$ and latent variable $z \sim \mathbf{N}(0, 1)$ as input to $G$, the output is $G(z, c) \sim p(d| c)$.

Following \citep{} \spnote{cite sgan}, the generator $G$ have the following components: 1. \textbf{Encoder}, which is a recurrent network that takes as input the past individual trajectories of the agents and generates independent representations, 2. \textbf{Pooling} module, that takes as input the representations of different humans next to each other and the relative positions, and generates a pooled representation which incooporates multi-agent interaction in our model, and 3. \textbf{Decoder}, a recurrent network which takes as input a latent variable $z$, the independent and pooled representations and generates a sample from the trajectory distribution prediction for the humans. Thus, using the generator $G$ and the latent variable $z \sim \mathcal{N}(0, 1)$, given the past trajectories of all humans $\tau_{0:t}^{1:n}$ we can generate samples for the future trajectories $\tau_{t:t+T}^{1:n}$ by approximation the distribution $p(\tau_{t:t+T}^{1:n}|\tau_{0:t}^{1:n}) \sim G(\tau_{0:t}^{1:n}, z)$. The discriminator $D$ is a recurrent neural network that takes as input a trajectory and predicts if its real or from the generator.

The generator $G$ and the discriminator $D$ are trained in a min-max game using the objective shown in Eq. \ref{eq:gan}. In order to model the distribution of trajectories, and diversity in samples from the generator, SGAN adds an auxillary variety loss, where it generates $k$ predictions and takes the L2 loss over the best prediction as the loss. This loss \cmnote{cite} encourages the network to produce diverse samples to model the different possible future trajectory given the past trajectory.
% \spnote{Describe the SGAN generator, pooling and discrimination model and training procedure}

We verified the effectiveness of the SGANs by comparing the prediction error across different baselines on two different types of datasets: 1. \textit{Offline} evaluation on the ETH/UCY Dataset, which is standard evaluation benchmark in literature and 2. \textit{Online} evaluation on a dataset of trajectories of humans and robot navigating next to each other in our lab. We also visualise the error in the form of error graphs, where we compare the error between the ground truth trajectories of the humans and the predicted trajectories for the humans as seen by the robot during navigation. More details regarding the dataset can be found in Sec \ref{}.

There are several reasons that we use SGANs over other probabilistic and deterministic models. Recent works on generating explicit distributions via Gaussian Processes \citep{SunM-RSS-21} involve modelling trajectories GPs, where the independent distributions are learned from human trajectory data. However, in order to generate joint trajectories distributions i.e. taking into account the effect of other agents on the given agents trajectory, \citep{} uses a cost function which maximizes the cooperation between the agents, and regularises deviation from the original distribution. However, since the pooling module $\mathcal{P}$ in SGANs, (which is responsible for jointly reasoning the future trajectory for all agents) is trained entirely from human demonstrations, it doesn't have any bias as it generated in a purely data driven mechanism. Recent works have also used inverse RL methods \citep{} to extract these cost functions from human data. However, they are computationally inefficient and cannot be used for real-time prediction of trajectories. SGANs provide us a data driven, real-time framework to generate samples from the joint future trajectory distribution of humans, and it is also invariant to the number of agents in the scene. Advancements in generative networks for trajectory prediction use extra information such as visual data \citep{} and flow data to generate more accurate predictions. However, in this work we consider only the trajectories of the agents and compare againsts similar baselines.


\spnote{Include table and graphs from the lab dataset; explain the baselines and the results from the offline datasets}



\begin{table}[]
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{Prediction Model} & \textbf{ETH-Uni}     & \textbf{Hotel}       & \textbf{Zara1}       & \textbf{Zara2}       & \textbf{UCY-Uni}     \\ \midrule
Linear Regression         & 0.58                 & 0.39                 & 0.44                 & 0.41                 & 0.6                  \\
MLP                       & 0.67                 & 1.59                 & 0.39                 & 0.38                 & 0.69                 \\
LSTM                      & 0.54                 & 2.91                 & 0.34                 & 0.43                 & 0.72                 \\
RED                       & 0.6                  & 0.47                 & 0.34                 & 0.31                 & 0.47                 \\
SR-LSTM                   & 0.63                 & 0.37                 & 0.41                 & 0.32                 & 0.51                 \\
CV                        & 0.58                 & 0.27                 & 0.34                 & 0.31                 & 0.46                 \\
CV-Noise                  & \textbf{0.43}        & \textbf{0.19}        & 0.24                 & 0.21                 & 0.34                 \\
ConstAcc                  & 1.35                 & 0.95                 & 0.59                 & 0.5                  & 0.79                 \\
SoPhie                    & 0.7                  & 0.76                 & 0.3                  & 0.38                 & 0.54                 \\
S-GAN                     & 0.59                 & 0.38                 & \textbf{0.18}        & \textbf{0.18}        & \textbf{0.26}        \\ \bottomrule
\end{tabular}
\caption{The average displacement error across different models on offline trajectory datasets.}
\label{tab:offline_ade}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{Prediction Model} & \textbf{ETH-Uni} & \textbf{Hotel} & \textbf{Zara1} & \textbf{Zara2} & \textbf{UCY-Uni} \\ \midrule
Linear Regression         & 1.11             & 0.81           & 0.93           & 0.83           & 1.19             \\
MLP                       & 1.32             & 3.12           & 0.81           & 0.77           & 1.38             \\
LSTM                      & 1.04             & 6.07           & 0.74           & 0.95           & 1.6              \\
RED                       & 1.14             & 0.94           & 0.76           & 0.7            & 1                \\
SR-LSTM                   & 1.25             & 0.74           & 0.9            & 0.7            & 1.1              \\
CV                        & 1.15             & 0.51           & 0.76           & 0.69           & 1.02             \\
CV-Noise                  & \textbf{0.8}     & \textbf{0.35}  & 0.48           & 0.45           & 0.71             \\
ConstAcc                  & 3.29             & 2.41           & 1.5            & 1.3            & 2.03             \\
SoPhie                    & 1.43             & 1.67           & 0.63           & 0.78           & 1.24             \\
S-GAN                     & 1.04             & 0.79           & \textbf{0.32}  & \textbf{0.34}  & \textbf{0.49}    \\ \bottomrule
\end{tabular}
\caption{The final displacement error across different models on offline trajectory datasets.}
\label{tab:offline_fde}
\end{table}


\begin{figure}
    \centering
    \begin{subfigure}{.98\linewidth}
     \centering
         \includegraphics[width = \linewidth]{figs/online_error.png}
        % \caption{Safety.} 
         \label{fig:safety-coop}
     \end{subfigure}
    % \begin{subfigure}{.48\linewidth}
    % \centering
    %     \includegraphics[width = \linewidth]{figs/coop_eff}
    %     \caption{Efficiency.}
    %     \label{fig:efficiency-real}
    % \end{subfigure}
\caption{Error in trajectory prediction of humans when the robot is navigating using the given prediction models in real-world experiments. Error bars indicate $95\%$ confidence intervals, and the line represents the minimum error across the samples which is common in literature. \label{fig:online-error-plots}}
\end{figure}



\begin{table}[]
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
Prediction Model & ADE            & FDE            \\ \midrule
SGAN-20          & \textbf{0.223} & \textbf{0.336} \\
SGAN-1           & 0.330          & 0.530          \\
CV               & 0.286          & 0.463          \\ \bottomrule
\end{tabular}
\caption{The average and the final displacement error in  online trajectory prediction of humans in real-world experiments.}
\label{tab:online_error}
\end{table}

Tables \ref{tab:offline_ade}, \ref{tab:offline_fde} compare the average and final displacement error in trajectory prediction across different offline datasets. \textit{SGAN} outperforms other baselines in terms of these metrics across most datasets. We observe that CV models with noise \cmnote{cite them}, work better across some datasets but in more complex datasets with more non-linear trajectories SGAN performs better.\spnote{verify claim!}

As shown in Table \ref{tab:online_error} we see that SGAN outperforms the baselines across the different datasets in terms of prediction error. We believe that as SGANs incorporate the past trajectories of humans and also the capture the interaction between different humans present in a scene to generate diverse samples, it is able to produce closer and more accurate predictions of human trajectories.

For real-world experiments(as explained in Section: \cmnote{add section}), the online error prediction is lower for SGAN-20 as compared to the other baselines tested in the real-world, as shown in the table \ref{tab:online_error}, and figure \ref{fig:online-error-plots}. \spnote{Need to explain the results and insights in more details??}


Recent work \spnote{cite them} has improved beyond the prediction qualities on such datasets even beyond SGANs. However, an important use of such high fidelity trajectory prediction models is in controllers for crowd navigation. In the further sections, we incorporate these different prediction models into a control framework for crowd navigation and investigate if the progress in prediction translates to an improvement in control and navigation. \spnote{Talk about why more recent models are complex + not real time in a single line} So, we believe SGANs serves a good prediction model which provide more accurate, real-time and diverse samples for predicting human trajectories.

\spnote{Add two line summary to just bring out everything}


% - Reason for using SGANs

% - Comparison over our dataset.




% - Existing methods
% - Deterministic
% - Probabilistic
% - Our approach: SGANs encoder decoder architecture
% - Comparison
% - Reason for choosing SGANs over others



% The goal is to jointly predict the future trajectory of all the $n$ humans navigating in the workspace, given the past trajectory. The positions of the agents in the workspace  $\mathcal{W}$ is denoted by position is denoted by $p^{i}$, where $p^i\in \mathcal{W}$, $\forall i \in\mathcal{N}=\{1, \dots, n\}$. The trajectory of an agent $i$ till time $t$ is denoted as $\tau_{\textbf{0:t}}^{i}$, and the future trajectory till time $T$ is represented as $\tau_{\textbf{t:t+T}}^{i}$, where $\tau_{\textbf{0:t}}^{i} = (p_{0}^{i}, \dots  p_{t}^{i})$, and $\tau_{\textbf{t:t+T}}^{i} = (p_{t}^{i}, \dots  p_{t+T}^{i})$. The model can be described as a function $f$ that maps the joint past trajectories $(\tau_{\textbf{0:t}} = \tau_{\textbf{0:t}}^{1}, \dots \tau_{\textbf{0:t}}^{n})$ to the joint future trajectories

% \begin{itemize}
%     \item Detail your prediction architecture
%     \item Show that your prediction works well in datasets (look at the table from "what constant velocity model can tell us...")
% \end{itemize}

% - Cost function not used
% - IRL work is not real time
% - Experimental results are key





% The probability distribution over the trajectories of an agent $i$ is denoted by $p^{i}(\tau^{i})$ and $p^{i}(\tau_{\textbf{t:t+T}}^{i} | \tau_{\textbf{0:t}}^{i}, \dots \tau_{\textbf{0:t}}^{n},)$ represents the conditional probability distribution over the future trajectory given past trajectory(s) of all agents $i\in\mathcal{N}$.
